Dig2DIG: Dig into Diffusion Information Gains for Image Fusion

Image fusion integrates complementary information from multi-source images to generate more informative results. Recently, the diffusion model, which demonstrates unprecedented generative potential, has been explored in image fusion. However, these approaches typically incorporate predefined multimodal guidance into diffusion, failing to capture the dynamically changing significance of each modality, while lacking theoretical guarantees. To address this issue, we reveal a significant spatio-temporal imbalance in image denoising; specifically, the diffusion model produces dynamic information gains in different image regions with denoising steps. Based on this observation, we Dig into the Diffusion Information Gains (Dig2DIG) and theoretically derive a diffusion-based dynamic image fusion framework that provably reduces the upper bound of the generalization error. Accordingly, we introduce diffusion information gains (DIG) to quantify the information contribution of each modality at different denoising steps, thereby providing dynamic guidance during the fusion process. Extensive experiments on multiple fusion scenarios confirm that our method outperforms existing diffusion-based approaches in terms of both fusion quality and inference efficiency.

==> sec/3_Preliminary.tex <==
%\section{Preliminary}
%这里是CCF的Preliminary+把扩散模型公式整理成要证明的形式。
%在DDPM（Denoising Diffusion Probabilistic Models）中，前向扩散会将干净样本 x0渐次加上噪声，最终变为近似高斯噪声。这个过程是线性的，因此在第 t步可以直接利用下面的离散闭式公式一次性采样xt而无需逐步迭代：
% In DDPM (Denoising Diffusion Probabilistic Models)~\cite{song2020denoising}, the forward diffusion process adds noise to a clean sample $x_0$ over multiple steps, eventually transforming it into nearly pure Gaussian noise. This procedure is linear, so one can sample $x_t$ in a single shot at step $t$ via the closed-form expression:
% \begin{equation}
% x_t = \sqrt{\bar{\alpha}_t} \, x_0 + \sqrt{1 - \bar{\alpha}_t} \, \epsilon, \quad \epsilon \sim \mathcal{N}(0, I),
% \label{eq:1}
% \end{equation}
% where $\alpha_t = 1 - \beta_t$, $\bar{\alpha}_t = \prod_{i=1}^t \alpha_i$, and $\{\beta_t\}_{t=1}^T$ is a predefined variance schedule. As $t$ increases, $x_t$ approaches a nearly pure noise distribution.

% To generate a sample during inference, one starts from pure noise $x_T$ and iteratively denoises down to $x_0$. Under a common parameterization, each reverse update step is given by:
% \begin{equation}
% x_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \, \epsilon_\theta(x_t, t) \right) + \sigma_\theta(t) \, z,
% \label{eq:2}
% \end{equation}
% where $\sigma_\theta^2(t) = \frac{(1 - \alpha_t)(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_t}$, $\epsilon_\theta(\cdot)$ is the network’s noise prediction, and $z \sim \mathcal{N}(0, I)$. By iterating from $t = T$ down to $t = 0$, one transforms pure noise into a nearly clean sample.

% From the closed-form forward process \cref{eq:1}, If the model $\epsilon_\theta(x_t, t)$ accurately predicts the noise $\epsilon$, one can approximate the “denoised” $\hat{x}_0$ as:
% \begin{equation}
% \hat{x}_0 = \frac{1}{\sqrt{\bar{\alpha}_t}} \left( x_t - \sqrt{1 - \bar{\alpha}_t} \, \epsilon_\theta(x_t, t) \right).
% \label{eq:3}
% \end{equation}
% This highlights the reverse denoising mechanism: once the correct noise component of $x_t$ is identified, we retrieve a good approximation of the clean data.

% From the perspective of stochastic differential equations or variational inference, and based on \cref{eq:1}, the gradient of \( \log p(x_t) \) with respect to \( x_t \) (i.e., the score function) can be expressed as:
% \begin{equation}
% \nabla_{x_t} \log p(x_t) = -\frac{x_t - \sqrt{\bar{\alpha}_t} x_0}{1 - \bar{\alpha}_t}. 
% \label{eq:4}
% \end{equation}
% Using the estimated \( \hat{x}_0 \) to replace \( x_0 \), and substituting Equation (3),into Equation (4), we derive:
% %准确来说，这里是约等于
% \begin{equation}
% \nabla_{x_t} \log p(x_t) = -\frac{\epsilon_\theta(x_t, t)}{\sqrt{1 - \bar{\alpha}_t}}. 
% \label{eq:5}
% \end{equation}
% In certain applications, such as text-to-image generation and multimodal data fusion, we often wish to incorporate additional conditions during the sampling process. By Bayes' theorem, the gradient of the conditional log-probability with respect to the current sample $x_t$ can be written as
% \begin{align}
% \nabla_{x_t} \log p(x_t \mid c)
% \;&=\; \nabla_{x_t} \log p(x_t) \notag \\
% &+\; \nabla_{x_t} \log p(c \mid x_t).
% \label{eq:6}
% \end{align}
% Here, $c$ represents one or more conditions guiding the generation process.

% For $K$ conditions $\{c_k\}_{k=1}^K$, assuming conditional independence given $x_t$, the joint log-probability can be expressed as:
% \begin{equation}
% \log p(c_1, \ldots, c_K \mid x_t)
% \;=\;
% \sum_{k=1}^K \log p(c_k \mid x_t).
% \label{eq:7}
% \end{equation}
% % Suppose we have $K$ individual conditions $\{c_k\}_{k=1}^K$ rather than a single $c$. If one assumes that these conditions are conditionally independent given $x_t$, then the joint conditional distribution factorizes as
% % \begin{equation}
% % p(c_1, c_2, \ldots, c_K \mid x_t)
% % \;=\;
% % \prod_{k=1}^K p(c_k \mid x_t),
% % \end{equation}
% % leading to
% % \begin{equation}
% % \log p(c_1, \ldots, c_K \mid x_t)
% % \;=\;
% % \sum_{k=1}^K \log p(c_k \mid x_t).
% % \end{equation}
% % Taking gradients with respect to $x_t$ then yields the \emph{exact} gradient sum:
% % \begin{equation}
% % \nabla_{x_t} \log p(c_1, \ldots, c_K \mid x_t)
% % \;=\;
% % \sum_{k=1}^K \nabla_{x_t} \log p(c_k \mid x_t).
% % \label{eq:exact_sum}
% % \end{equation}
% In practice, however, these conditions may not be strictly independent, or we may wish to control the influence of each individual condition. Hence, instead of the strict equality in \cref{eq:7}, one frequently uses a weighted approximation:
% \begin{equation}
% \nabla_{x_t} \log p(c \mid x_t)
% \;\approx\;
% \sum_{k=1}^K w_k \,\nabla_{x_t} \log p(c_k \mid x_t),
% \label{eq:8}
% \end{equation}
% where $w_k$ is a user-defined weight indicating the relative importance of condition $c_k$. Substituting \cref{eq:8} into \cref{eq:6} then gives:
% \begin{align}
% \nabla_{x_t} \log p(x_t \mid c)
% \;&\approx\;
% \nabla_{x_t} \log p(x_t) \notag \\
% &+\;
% \sum_{k=1}^K w_k \,\nabla_{x_t} \log p(c_k \mid x_t).
% \label{eq:9}
% \end{align}
% By adjusting the weights $\{w_k\}$, one can modulate the strength of each condition's contribution to the gradient-based sampling step, thus allowing fine-grained control over the generated samples.
% %长版
% % \begin{align}
% % x_{t-1}
% % &=\;
% % \frac{1}{\sqrt{\alpha_t}}
% % \biggl[
% %   x_t 
% %   \;-\;
% %   \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}}
% %   \Bigl(
% %    -\sqrt{1 - \bar{\alpha}_t}\,\bigl(\nabla_{x_t} \log p(x_t \mid c) 
% %      \;-\;\sum_{k=1}^K w_k\,\nabla_{x_t} \log p(c_k \mid x_t)\bigr)
% %   \Bigr)
% % \biggr]
% % \;+\;
% % \sigma_\theta(t)\,z
% % \\[6pt]
% % &=\;
% % \frac{1}{\sqrt{\alpha_t}}
% % \Bigl[
% %   x_t 
% %   \;+\;
% %   \bigl(1 - \alpha_t\bigr)\,\nabla_{x_t}\log p(x_t \mid c) 
% %   \;-\;
% %   \bigl(1 - \alpha_t\bigr)\sum_{k=1}^K w_k\,\nabla_{x_t} \log p(c_k \mid x_t)
% % \Bigr]
% % \;+\;
% % \sigma_\theta(t)\,z.
% % \end{align}

% %短版
% % \begin{align}
% % x_{t-1}
% % &=\;
% % \frac{1}{\sqrt{\alpha_t}}
% % \Bigl[
% %   x_t 
% %   \;+\;
% %   \bigl(1 - \alpha_t\bigr)\,\nabla_{x_t}\log p(x_t \mid c) 
% %   \;-\;
% %   \bigl(1 - \alpha_t\bigr)\sum_{k=1}^K w_k\,\nabla_{x_t} \log p(c_k \mid x_t)
% % \Bigr]
% % \;+\;
% % \sigma_\theta(t)\,z.
% % \end{align}
% From \cref{eq:2}, \cref{eq:5}, and \cref{eq:9}, we derive the following update equation for the diffusion model:
% \begin{align}
% x_{t-1} 
% &=
% \frac{1}{\sqrt{\alpha_t}} x_t \notag \\
% &
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\nabla_{x_t} \log p(x_t)}_{\text{Unconditional Guidance}} \notag \\
% &
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\sum_{k=1}^K w_k \nabla_{x_t} \log p(c_k \mid x_t)}_{\text{Multimodal Guidance}} \notag \\
% &
% +\underbrace{\sigma_\theta(t) z}_{\text{Noise}}.
% \label{eq:10}
% \end{align}
% This equation demonstrates that the update step in the diffusion model can be decomposed into three key components: Unconditional Guidance, Multimodal Guidance, and Noise.
% This decomposition encourages further exploration of the role of Multimodal Guidance in reducing the model's generalization error and improving conditional generation quality.

% \section{Preliminary}

% In DDPM~\cite{song2020denoising}, a clean sample $x_0$ gradually transitions to nearly pure noise via the forward diffusion process:
% \begin{equation}
% x_t = \sqrt{\bar{\alpha}_t} \, x_0 + \sqrt{1 - \bar{\alpha}_t} \, \epsilon, 
% \quad \epsilon \sim \mathcal{N}(0, I),
% \label{eq:1}
% \end{equation}
% where $\bar{\alpha}_t = \prod_{i=1}^t (1-\beta_i)$. During inference, one iteratively denoises from noise $x_T$ back to $x_0$ via
% \begin{equation}
% x_{t-1} = \frac{1}{\sqrt{\alpha_t}} \Bigl( x_t 
% - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \, \epsilon_\theta(x_t, t)\Bigr) 
% + \sigma_\theta(t)\,z,
% \label{eq:2}
% \end{equation}
% where $\sigma_\theta^2(t) = \frac{(1 - \alpha_t)(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_t}$.

% If $\epsilon_\theta$ accurately predicts $\epsilon$, we obtain
% \begin{equation}
% \hat{x}_0 
% = 
% \frac{1}{\sqrt{\bar{\alpha}_t}}
% \Bigl[
%   x_t \;-\; \sqrt{1 - \bar{\alpha}_t}\,\epsilon_\theta(x_t, t)
% \Bigr].
% \label{eq:3}
% \end{equation}
% From \cref{eq:1}, the gradient of $\log p(x_t)$ satisfies
% \begin{equation}
% \nabla_{x_t} \log p(x_t) 
% =
% -\frac{x_t - \sqrt{\bar{\alpha}_t}\,x_0}{1 - \bar{\alpha}_t}.
% \label{eq:4}
% \end{equation}
% Replacing $x_0$ with $\hat{x}_0$ yields
% \begin{equation}
% \nabla_{x_t} \log p(x_t) 
% \approx 
% -\frac{\epsilon_\theta(x_t, t)}{\sqrt{1 - \bar{\alpha}_t}}.
% \label{eq:5}
% \end{equation}

% In many conditional tasks, we adjust the generation with conditions $c$. By Bayes' rule,
% \begin{align}
% \nabla_{x_t}\log p(x_t \mid c)
% &=
% \nabla_{x_t}\log p(x_t)
% \;+\;
% \nabla_{x_t}\log p(c\mid x_t).
% \label{eq:6}
% \end{align}
% For $K$ conditions $\{c_k\}$, one often uses a weighted approximation:
% \begin{equation}
% \nabla_{x_t} \log p(c \mid x_t)
% \;\approx\;
% \sum_{k=1}^K w_k \,\nabla_{x_t} \log p(c_k \mid x_t),
% \label{eq:8}
% \end{equation}
% leading to
% \begin{equation}
% \nabla_{x_t}\log p(x_t \mid c)
% \;\approx\;
% \nabla_{x_t}\log p(x_t)
% \;+\;
% \sum_{k=1}^K w_k \,\nabla_{x_t}\log p(c_k \mid x_t).
% \label{eq:9}
% \end{equation}
% Combining \cref{eq:2}, \cref{eq:5}, and \cref{eq:9} produces the update:
% \begin{align}
% x_{t-1} 
% &=
% \frac{1}{\sqrt{\alpha_t}} x_t 
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\nabla_{x_t} \log p(x_t)}_{\text{Unconditional Guidance}} 
% \notag\\
% &\quad
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\sum_{k=1}^K w_k\, \nabla_{x_t} \log p(c_k \mid x_t)}_{\text{Multimodal Guidance}}
% +\underbrace{\sigma_\theta(t)\,z}_{\text{Noise}}.
% \label{eq:10}
% \end{align}
% These terms reveal how unconditional and conditional guidance jointly shape the denoising trajectory in diffusion models.




% % 省略了部分推导和证明，完整内容请参见附录

% % 原文开始
% %这里是CCF的Preliminary+把扩散模型公式整理成要证明的形式。
% %在DDPM（Denoising Diffusion Probabilistic Models）中，前向扩散会将干净样本 x0渐次加上噪声，最终变为近似高斯噪声。这个过程是线性的，因此在第 t步可以直接利用下面的离散闭式公式一次性采样xt而无需逐步迭代：
% In DDPM (Denoising Diffusion Probabilistic Models)~\cite{song2020denoising}, the forward diffusion process adds noise to a clean sample $x_0$ over multiple steps, eventually transforming it into nearly pure Gaussian noise. This procedure is linear, so one can sample $x_t$ in a single shot at step $t$ via the closed-form expression:
% \begin{equation}
% x_t = \sqrt{\bar{\alpha}_t} \, x_0 + \sqrt{1 - \bar{\alpha}_t} \, \epsilon, \quad \epsilon \sim \mathcal{N}(0, I),
% \label{eq:1}
% \end{equation}
% where $\alpha_t = 1 - \beta_t$, $\bar{\alpha}_t = \prod_{i=1}^t \alpha_i$, and $\{\beta_t\}_{t=1}^T$ is a predefined variance schedule. As $t$ increases, $x_t$ approaches a nearly pure noise distribution.

% To generate a sample during inference, one starts from pure noise $x_T$ and iteratively denoises down to $x_0$. Under a common parameterization, each reverse update step is given by:
% \begin{equation}
% x_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \, \epsilon_\theta(x_t, t) \right) + \sigma_\theta(t) \, z,
% \label{eq:2}
% \end{equation}
% where $\sigma_\theta^2(t) = \frac{(1 - \alpha_t)(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_t}$, $\epsilon_\theta(\cdot)$ is the network’s noise prediction, and $z \sim \mathcal{N}(0, I)$.

% From the closed-form forward process \cref{eq:1}, if the model $\epsilon_\theta(x_t, t)$ accurately predicts the noise $\epsilon$, one can approximate the “denoised” $\hat{x}_0$ as:
% \begin{equation}
% \hat{x}_0 = \frac{1}{\sqrt{\bar{\alpha}_t}} \left( x_t - \sqrt{1 - \bar{\alpha}_t} \, \epsilon_\theta(x_t, t) \right).
% \label{eq:3}
% \end{equation}
% This reveals the reverse denoising mechanism: once the noise part of $x_t$ is identified, we recover an approximate clean sample.

% From \cref{eq:1}, the gradient of $ \log p(x_t) $ satisfies:
% \begin{equation}
% \nabla_{x_t} \log p(x_t) = -\frac{x_t - \sqrt{\bar{\alpha}_t} x_0}{1 - \bar{\alpha}_t}, 
% \label{eq:4}
% \end{equation}
% and replacing $ x_0 $ with $ \hat{x}_0 $ yields (approximately):
% \begin{equation}
% \nabla_{x_t} \log p(x_t) = -\frac{\epsilon_\theta(x_t, t)}{\sqrt{1 - \bar{\alpha}_t}}. 
% \label{eq:5}
% \end{equation}

% In many conditional tasks, conditions $c$ can be incorporated. By Bayes' theorem,
% \begin{align}
% \nabla_{x_t} \log p(x_t \mid c)
% \;&=\; \nabla_{x_t} \log p(x_t) \notag \\
% &+\; \nabla_{x_t} \log p(c \mid x_t),
% \label{eq:6}
% \end{align}
% and for $K$ conditions $\{c_k\}_{k=1}^K$, a weighted approximation is often used:
% \begin{equation}
% \nabla_{x_t} \log p(c \mid x_t)
% \;\approx\;
% \sum_{k=1}^K w_k \,\nabla_{x_t} \log p(c_k \mid x_t),
% \label{eq:8}
% \end{equation}
% leading to
% \begin{align}
% \nabla_{x_t} \log p(x_t \mid c)
% \;&\approx\;
% \nabla_{x_t} \log p(x_t) \notag \\
% &+\;
% \sum_{k=1}^K w_k \,\nabla_{x_t} \log p(c_k \mid x_t).
% \label{eq:9}
% \end{align}
% By adjusting $\{w_k\}$, one can control the influence of each condition.

% Using \cref{eq:2}, \cref{eq:5}, and \cref{eq:9}, we derive the diffusion update:
% \begin{align}
% x_{t-1} 
% &=
% \frac{1}{\sqrt{\alpha_t}} x_t \notag \\
% &
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\nabla_{x_t} \log p(x_t)}_{\text{Unconditional Guidance}} \notag \\
% &
% +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\sum_{k=1}^K w_k \nabla_{x_t} \log p(c_k \mid x_t)}_{\text{Multimodal Guidance}} \notag \\
% &
% +\underbrace{\sigma_\theta(t) z}_{\text{Noise}}.
% \label{eq:10}
% \end{align}
% This demonstrates that the update step consists of Unconditional Guidance, Multimodal Guidance, and Noise, offering flexible control over conditional generation.
\section{Methods}
\label{sec:prelim_short}

In Denoising Diffusion Probabilistic Models (DDPM)~\cite{song2020denoising}, the forward diffusion process gradually adds noise to a clean sample $x_0$ until it becomes nearly Gaussian. This step can be sampled directly via:
\begin{equation}
x_t = \sqrt{\bar{\alpha}_t}\, x_0 + \sqrt{1 - \bar{\alpha}_t}\,\epsilon,\quad \epsilon \sim \mathcal{N}(0, I),
\label{eq:1}
\end{equation}
where $\alpha_t = 1 - \beta_t$, $\bar{\alpha}_t = \prod_{i=1}^t \alpha_i$, and $\{\beta_t\}$ is a predefined variance schedule.

During inference, one starts from noise $x_T$ and iteratively denoises via the reverse update:
\begin{equation}
x_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}}\, \epsilon_\theta(x_t, t) \right) + \sigma_\theta(t)\, z,
\label{eq:2}
\end{equation}
where $\sigma_\theta^2(t) = (1 - \alpha_t)(1 - \bar{\alpha}_{t-1})/(1 - \bar{\alpha}_t)$, $\epsilon_\theta(\cdot)$ is the network’s noise prediction, and $z \sim \mathcal{N}(0,I)$.

From the forward process, if $\epsilon_\theta$ accurately reflects the noise in $x_t$, one can approximate the score function (the gradient of $\log p(x_t)$) as:
\begin{equation}
\nabla_{x_t}\! \log p(x_t) = -\frac{\epsilon_\theta(x_t, t)}{\sqrt{1 - \bar{\alpha}_t}}.
\label{eq:5}
\end{equation}

In many tasks, we also incorporate conditions $c$, each contributing an additional gradient. A practical weighted approximation of the conditional gradient is:
\begin{align}
\nabla_{x_t}\! \log p(x_t \mid c)
&\approx
\nabla_{x_t}\! \log p(x_t)
\notag \\
&\quad+
\sum_{k=1}^K w_k \,\nabla_{x_t}\! \log p(c_k \mid x_t).
\label{eq:9}
\end{align}

Combining \eqref{eq:2}, \eqref{eq:5}, and \eqref{eq:9} gives the final update step:
\begin{align}
x_{t-1}
&= \frac{1}{\sqrt{\alpha_t}} x_t+\underbrace{\sigma_\theta(t)\, z}_{\text{Noise}}
+\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\nabla_{x_t}\! \log p(x_t)}_{\text{Unconditional Guidance}}
\notag \\
& \quad +\underbrace{\frac{1}{\sqrt{\alpha_t}} (1 - \alpha_t)\sum_{k=1}^K w_k \nabla_{x_t}\! \log p(c_k \mid x_t)}_{\text{Multimodal Guidance}}
\label{eq:10}
\end{align}

This succinctly shows how an unconditional term, multimodal guidance, and random noise jointly shape the sample at each reverse step. For full derivations and additional details, see Appendix.
